Proxy Methods for Domain Adaptation

We study the problem of domain adaptation under distribution shift, where the shift is due to a change in the distribution of an unobserved, latent variable that confounds both the covariates and the labels. In this setting, neither the covariate shift nor the label shift assumptions apply. Our approach to adaptation employs proximal causal learning, a technique for estimating causal effects in settings where proxies of unobserved confounders are available. We demonstrate that proxy variables allow for adaptation to distribution shift without explicitly recovering or modeling latent variables. We consider two settings, (i) Concept Bottleneck: an additional ''concept'' variable is observed that mediates the relationship between the covariates and labels; (ii) Multi-domain: training data from multiple source domains is available, where each source domain exhibits a different distribution over the latent confounder. We develop a two-stage kernel estimation approach to adapt to complex distribution shifts in both settings. In our experiments, we show that our approach outperforms other methods, notably those which explicitly recover the latent confounder.

==> sections/3_2_theory_partial.tex <==
\subsection{Identification with Only Proxies}
There might be conditions that $C$ is not observed in the target domain as labeling concepts takes extra efforts in many machine learning applications. In such scenario, although Theorem~\ref{theorem:complete_identification} can not be applied, we show that partial identification is possible when $C$ is a deterministic function of $U$ and $X$. with the help of proxy variable $W$. This is motivated by single proxy control~\citep{tchetgen2014control, tchetgen2023single} that introduces a new bridge function developed to estimate the causal effect with single proxy. To show the identifiability result, it requires the deterministic assumption.
%When $C$ is unobserved, we are able identify the conditional distribution of $C$ given $x$ with the proxy variable $W$. This allows us to partially identify the distribution of $\EE_q[Y\mid x]$. 
\begin{assumption}[Deterministic Confounding]\label{assumption:deterministicC}
There exists a deterministic function $\gamma_0$ such that $C=\gamma_0(X,U)$ and $\EE\norm{\gamma_0(x,U)}<\infty$ for all $x\in\Xcal$. 
\end{assumption}
For both $f\in\{q,p\}$, we define the bridge function $m_0^f$ that satisfies the followings:
\begin{align*}
1 &= \int_{\Wcal}{m}_0^f(w,c,x)f(w\mid c,x)dw; \\
p(c\mid x)&=\int_{\Wcal}{m}_0^f(w,c,x)p(w\mid x)dw.
\end{align*}
%It is easy to see that one possible solution for $m_0^f(w,c,x)$ is %$f(c\mid w,x)$. However, this bridge function is not domain invariant as
%$$f(c\mid w,x)=\frac{\int p(c\mid x, u)p(w,x\mid u)f(u)du}{\int p(w, x\mid u)f(u)du},$$ differs across domains. Hence this bridge function is not transferable as $h_0$ does without additional condition. The following condition is a sufficient condition for the bridge function $m_0$ to be domain invariant. 

Under Assumption~\ref{assumption:CI}--\ref{assumption:completeness}, \ref{assumption:deterministicC} and additional regularity conditions stated in Appendix~\ref{appendix:existemce_m0}, the solution of $m_0^f$ for $f\in\{p,q\}$ exists as shown in Appendix~\ref{appendix:existemce_m0}. Our goal is to show that all solutions of $m_0^f$ are invariant across domains.  
%similar to~\eqref{eq:h0}. For both the source domain and target domain, $f\in\{p,q\}$, we define
%\[
%f(c\mid u,x)=\int_{\Wcal}m_0^f(w,c,x)f(w\mid u)dw.
%\]
% Under Assumption~\ref{assumption:graph}, it is easy to see that $m_0^p=m_0^q$ almost surely with respect to $p(w\mid u)$ for $u\in\Ucal$. Hence, $m_0:=m_0^p$ is transferable to the target domain. We show that $m_0^f,f\in\{p,q\}$ exist under the regularity conditions~\ref{assumption:completeness:action}--\ref{assumption:compactness} in Proposition~\ref{prop:existence_m0}.

\begin{theorem}\label{theorem:partial_iden}
Under Assumption~\ref{assumption:graph}--\ref{assumption:deterministicC} and additional reularity conditions xxx stated in Appendex~\ref{appendix:existemce_m0}, we have  
\[
q(c\mid x)=\int_{\Wcal}m_0^p(w,c,x)q(w\mid x)dw.
\]
Given $(W,X,C,Y)$ from the source and $(W,X)$ from the target and assume that $h_0^f$ for $f\in\{p,q\}$ exist, $m_0^p, h_0^p, q(w\mid x)$ are identifiable. 
Additionally, define $r_{x}^q(w,c)=q(w,c\mid x)/q(w\mid  x)q(c\mid x)$ be the conditional copula density of the target domain, 
we can partially identify $\EE_q[Y\mid x]$ as 
\[
\int_{\Wcal\Ccal}h_0^p(w,c)q_{m_0}(c\mid x)q(w\mid x)r^q_x(w,c)dcdw,
\]
where $q_{m_0}(c\mid x)=\int_{\Wcal}m_0^p(w,x,c)q(w\mid x)dw$.
\end{theorem}
The component that is unidentifiable is $r_{x}^q(w,c)$, which quantifies the degree of dependency of $W$ and $C$ given $x$. 
%If $\sup_{w,c}|q(w,c\mid x)-q(w\mid x)q(c\mid x)|<\delta_x$ for some small $\delta_x>0$, we might expect $\EE_q[Y\mid x]\approx \int_{\Wcal}\int_{\Ccal}h_0^p(w,c)q(c\mid x)q(w\mid x)dcdw$. 
Under this setting, an interesting question is to find the range of all possible $\EE_q[Y\mid x]$. It is easy to see that $r_x^q(w,c)\leq \min(1/q(w\mid x), 1/q(c\mid x))$ and hence an nontrivial upper bound can be obtained so long as $q(w\mid x), q(c\mid x)>0$. If we have prior information about copula density, e.g., the range of correlation in the Gaussian case, we might be able to obtain a tighter bound. 
We provide two examples, a discrete case and a continuous case, in the following to show that tighter bounds can be obtained in some cases. 
\begin{example}[Bernoulli Case]
\begin{table}
    \centering
    \begin{tabular}{c|c|c|c}
    &$W=0$&$W=1$&\\
    \hline
    $C=0$ & $q_{00\mid x}$ & $q_{01\mid x}$ & $1-\pi_{C\mid x}$ \\
    \hline
    $C=1$&$q_{10\mid x}$&$q_{11\mid x}$&$\pi_{C\mid x}$\\
    \hline
    &$1-\pi_{W\mid x}$&$\pi_{W\mid x}$&
    \end{tabular}
    \caption{Conditional probabilities of $W,C$ given $x$.}
    \label{tab:prob}
\end{table}
We study the case where $W,C$ are binary variables and write $
\EE_q[Y\mid x] = \sum_{w,c=0}^1 h_0(w,c)q(w,c\mid x)$.
%where the conditional marginals are known. 
Define $\pi_{W\mid x}=q(W=1\mid x)$ and $\pi_{C\mid x}=q(C=1\mid x)$. Using the result from Table~\ref{tab:prob}, we can write $\EE_q[Y\mid x]$ as
\begin{multline}\label{eq:Ey_x}
    h_0(0,0)(1-\pi_{C\mid x}-\pi_{W\mid x}) + h_0(0,1)\pi_{W\mid x} + h_0(1,0)\pi_{C\mid x}\\
    + q_{11\mid x}\{h_0(0,0)-h_0(0,1)-h_0(1,0)+h_0(1,1)\}.
\end{multline}
Here the only unknown is $q_{11\mid x}$. We can apply Fr\'echet–Hoeffding bound on $q_{11\mid x}$ and obtain
\[
\max(0,\pi_{C\mid x}+\pi_{W\mid x}-1)\leq q_{11\mid x}\leq \min(\pi_{C\mid x},\pi_{W\mid x}).
\]
Plug the result into~\eqref{eq:Ey_x}, we can obtain the upper and lower bound of $\EE_q[Y\mid x]$. 
\end{example}
The example can be extended beyond binary random variables to categorical random variables by applying Fr\'echet–Hoeffding bound. In the next example, we study the Gaussian linear case.  
\begin{example}[Gaussian Linear Case] Let  $E,D, F, A, G$ be matrices, $\Sigma_U,\Psi_X, \Psi_W,\Psi_C,\Psi_Y$ be positive definite matrices, and $D$ is invertible. The noise random variables $\varepsilon_x, \varepsilon_w, \varepsilon_c, \varepsilon_y$ are pairwise independent and independent of $U$. Additionally $\varepsilon_c$ is independent of $X$ and $\varepsilon_y$ is independent of $C$. 
\begin{align*}
U&\sim\mathcal{N}(0,\Sigma_U);\\
X &= EU + \varepsilon_x,\quad\varepsilon_x\sim\mathcal{N}(0,\Psi_X);\\
W &= DU + \varepsilon_w,\quad\varepsilon_w\sim\mathcal{N}(0,\Psi_W);\\
C &= FX + GU + \varepsilon_c,\quad\varepsilon_c\sim\mathcal{N}(0,\Psi_C);\\
Y &= U^\top A C + \varepsilon_y,\quad\varepsilon_y\sim\mathcal{N}(0,\Psi_Y).
\end{align*}
By algebraic manipulation, the bridge function is $h_0(w,c)=w^\top H c$ with $H=D^{-1}A$. Define $$R_{CW\mid x}=\begin{bmatrix}I&\Sigma_{W\mid x}^{-1/2}\Sigma_{WC\mid x}\Sigma_{C\mid x}^{-1/2}\\ \Sigma_{C\mid x}^{-1/2}\Sigma_{CW\mid x}\Sigma_{W\mid x}^{-1/2}&I\end{bmatrix},$$ as the correlation matrix and $\tilde{H} = \Sigma_{W\mid X}^{1/2}H\Sigma_{C\mid X}^{1/2}$
Hence, by algebraic manipulation, we have
\[
E_{R}[Y\mid x]=\mu_{W\mid x}^\top H\mu_{C\mid x}+tr(R_{CW\mid x}\tilde{H}).
\]
Here the only unknown is $R_{CW\mid x}$. Using the fact that $\norm{R_{CW\mid x}}\leq 1$, we can obtain the upper and lower bound as $\mu_{W\mid x}^\top H\mu_{C\mid x}\pm \sum_i\sigma_i(\tilde{H})$. If we have additional information about the upper bound of correlation $\norm{R_{CW\mid x}}\leq\rho\leq 1$, a tighter bound $\mu_{W\mid x}^\top H\mu_{C\mid x}\pm \sum_i\rho\sigma_i(\tilde{H})$ is achieved. 
\end{example}
We demonstrate that this bound is tight empirically by running the simulations in Appendix. The bridge function we study is a quadratic function with respect to $C$ and $W$. For the Gaussian distribution, in general, we are able to obtain nontrivial sensitivity bound when $h_0$ can be well-approximated by second-order Taylor expansion. More discussion is in Appendix~\ref{sec:sensitivity_analysis}. 




==> sections/4_2_kernel_partial.tex <==
\subsection{Kernel bridge function $m_0$}
In the absence of the concept variable $C$, as an alternative to~\eqref{eq:full_e}, we apply the Theorem~\ref{theorem:partial_iden} to estimate the conditional marginal $q(c\mid x)$ and construct the following predictor
\begin{equation}\label{eq:front_e}
y_{\text{partial}}(x)=\dotp{h_0}{\mu_{W\mid x}^q\otimes\mu_{C\mid x}^q}.
\end{equation}
Our approach is to use the bridge function $m_0$ introduced in Section~\ref{ssec:identification} and compute the conditional distribution with the proxy $W$. Suppose that $m_0\in\Hcal_{\Wcal\Ccal\Xcal}$ and recall $q(c|x)=\int m(w,c,x)q(w\mid x)dw$, we can express $\mu_{C\mid x}^q$ as
\begin{align}\label{eq:cme_m0}
\mu_{C\mid x}^q &=\int \phi(c)\int m(w,c,x)q(w\mid x)dwdc\notag\\
&= \int\phi(c)\dotp{m_0}{\mu_{W\mid x}^q\otimes\phi(c)\otimes\phi(x)}dc
\end{align}
From~\eqref{eq:cme_m0}, we see that a more direct method to compute $\mu_{C\mid x}^q$ is to construct a conditional mean embedding that embeds the bridge function $m_0$. To this end, we define the operator $A:\Hcal_{\Wcal\Xcal}\rightarrow\Hcal_\Ccal$ as
\begin{equation}\label{eq:defineA}
A[\mu_{W\mid x}^q\otimes\phi(x)]=\int\phi(c)\dotp{m_0}{\mu_{W\mid x}^q\otimes\phi(c)\otimes\phi(x)}dc.
\end{equation}
We call this construction as the \emph{double conditional mean embedding} as it takes $\mu_{W\mid x}^p$ as a embedding to construct another embedding $\mu_{C\mid x}^q$. It is easy to see that the operator $A$ is invariant across domains as $m_0$ is invariant across domains: $\mu_{C\mid x}^p=A[\mu_{W\mid x}^p\otimes\phi(x)]$ for any $x\in\Xcal$. Hence, to adapt the distribution shift, a natural next step is to estimate $A$ from the source domain.
 We take the approach developed in~\citep{grunewalder2012conditional} that shows the estimation of conditional mean embedding is equivalent as solving a linear regression problem. We apply this idea and consider the following empirical risk. Let $\hat{\mu}_{W\mid x}^p$ be the empirical estimate of $\mu_{W\mid x}^p$ using i.i.d. samples $(W_3, X_3)=\{(w_{3,i}, x_{3,i})\}_{i=1}^{n_3}$ from source with regularization parameter $\lambda_3>0$. 
 Let $\lambda_4>0$, $(C_4, X_4)=\{(c_{4,i}, x_{4,i})\}_{i=1}^{n_4}$ be i.i.d. samples from the source, we want to minimize
 \begin{multline}\label{eq:doublekemb_erm}
      \frac{1}{2n_4}\sum_{i=1}^{n_4}\|\phi(c_{4,i})-A[\hat{\mu}_{W\mid x_{4,i}}^p \otimes \phi(x_{4,i})]\|_{\Hcal_C}^2\\+\frac{\lambda_4}{2}\opnorm{A}{\Hcal_{\Wcal\Xcal}}^2,
\end{multline}
where the optimal solution is presented in the following proposition.  
\begin{proposition}\label{prop:optimal_m0}
Define $\Kcal_{X_3}\in\RR^{n_3\times n_3}$, $\Kcal_{X_4}\in\RR^{n_4\times n_4}$, $\Kcal_{W_3}\in\RR^{n_3\times n_3}$,  $\Kcal_{X_{34}}\in\RR^{n_3\times n_4}$ be the Gram matrices of $X_3$, $X_4$, $W_3$, and $(X_3,X_4)$ respectively. Let $\Phi_{X_3}$, $\Phi_{C_4}$ be the vectorized feature maps of $X_3$, and $C_4$ respectively. Let $\Phi_{\hat{\mu}_{{W}\mid X_3}}=(\dotp{\hat{\mu}_{{W}\mid x_{3,1}}}{\cdot}\cdots \dotp{\hat{\mu}_{{W}\mid x_{3,n_3}}}{\cdot})^\top\in\Hcal_W^{n_3}$. Then, the optimal solution to~\eqref{eq:doublekemb_erm} is
\[
\hat{A}=\Phi_{C_4}^\top(\tilde{\Kcal}+\lambda_4I)^{-1}(\Phi_{X_3}\odot\Phi_{\hat{\mu}_{{W}\mid X_3}}),
\]
where $\tilde{\Kcal}=\Kcal_{X_4}\odot\{ \Kcal_{X_{43}}(\Kcal_{X_3}+\lambda_3 I)^{-1}\Kcal_{W_3}(\Kcal_{X_3}+\lambda_3 I)\Kcal_{X_{34}}\}$.
\end{proposition}
Therefore, given a new sample $x_{\text{new}}$ the empirical version of~\eqref{eq:front_e} is
\[
\hat{y}_{\text{partial}}(x_{\text{new}})=\dotp{\hat{h}_0}{\hat{A}[\hat{\mu}_{W\mid x_{\text{new}}}^q\otimes \phi(x_{\text{new}})]\otimes\hat{\mu}_{W\mid x_{\text{new}}}^q}.
\]
Then, we complete the partial adaptation procedure. 

==> sections/99_scratch.tex <==
% This is relevant when it is of interest to develop a model using data collected in one context and deploy it in related context (e.g., for data collected at a later time or from a different location) for which resource or other constraints limit the availability of labeled data.
% For example, in applications of machine learning in healthcare, a diagnostic or prognostic model developed using data from one hospital might perform poorly when applied to data collected from another due to differences in patient population or differences in patterns of data collection or care delivery. 
% with a different patient population or with different practices for care delivery or data collection.
% Labeled data may be unavailable in a target domain for several reasons including resource constraints that limit annotation or limited observation of long-term outcomes in prognostic settings.
% It is motivated by the fact that labeling data is often labor intensive and requires domain expertise. 
% Additionally, the underlying distributions might change when data are collected in different environments, times, or locations~\citep{koh2021wilds, malinin2021shifts}. 
% For example, the distribution of patients diagnosed with skin cancer from hospital $A$ and hospital $B$ might be different due to patients’ socioeconomic status, demographics, and other factors. 
% However, we might only have the labeled data from hospital $A$, and just unlabeled data from hospital $B$ (e.g., hospital $B$ may have less funding). 
% If we were to train an accurate model on patients from hospital $A$ and apply it on patients from hospital $B$, it may perform poorly on this different distribution.

==> sections/checklist.tex <==
\newpage
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references. For each question, choose your answer from the three possible options: Yes, No, Not Applicable.  You are encouraged to include a justification to your answer, either by referencing the appropriate section of your paper or providing a brief inline description (1-2 sentences). 
%Please do not modify the questions.  Note that the Checklist section does not count towards the page limit. Not including the checklist in the first submission won't result in desk rejection, although in such case we will ask you to upload it during the author response period and include it in camera ready (if accepted).

%\textbf{In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.}
% %%% END INSTRUCTIONS %%%


 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [No]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes]
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [No] We are planning to release the code upon publication.
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Yes]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Yes]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Yes]
   \item The license information of the assets, if applicable. [Yes]
   \item New assets either in the supplemental material or as a URL, if applicable. [Not Applicable]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}

